Variety of disc wind-driven explosions in massive rotating stars. II. Dependence on the progenitor

We assess the variance of supernova(SN)-like explosions associated with the core collapse of rotating massive stars into a black hole-accretion disc system under changes in the progenitor structure. Our model of the central engine evolves the black hole and the disc through the transfer of matter and angular momentum and includes the contribution of the disc wind. We perform two-dimensional, non-relativistic, hydrodynamics simulations using the open-source hydrodynamic code Athena++, for which we develop a method to calculate self-gravity for axially symmetric density distributions. For a fixed model of the wind injection, we explore the explosion characteristics for progenitors with zero-age main-sequence masses from 9 to 40 $M_\odot$ and different degrees of rotation. Our outcomes reveal a wide range of explosion energies with $E_\mathrm{expl}$ spanning from $\sim 0.3\times10^{51}$~erg to $ > 8\times 10^{51}$~erg and ejecta mass $M_\mathrm{ej}$ from $\sim 0.6$ to $> 10 M_\odot$. Our results are in agreement with some range of the observational data of stripped-envelope and high-energy SNe such as broad-lined type Ic SNe, but we measure a stronger correlation between $E_\mathrm{expl}$ and $M_\mathrm{ej}$. We also provide an estimate of the $^{56}$Ni mass produced in our models which goes from $\sim0.04\;M_\odot$ to $\sim 1.3\;M_\odot$. The $^{56}$Ni mass shows a correlation with the mass and the angular velocity of the progenitor: more massive and faster rotating progenitors tend to produce a higher amount of $^{56}$Ni. Finally, we present a criterion that allows the selection of a potential collapsar progenitor from the observed explosion energy.

==> old_table.tex <==
\begin{tabular}{c|ccccccccc}
\hline\hline
model & $E_\mathrm{inj}$ & $M_\mathrm{ej}$ & $E_\mathrm{expl}$ & $v_\mathrm{ej}$ & $N_\mathrm{p}$ & $M_\mathrm{ej}^\mathrm{inj}$ & $M_\mathrm{ej,>5GK}$ ($N_\mathrm{ej,>5GK}$) & $M^\mathrm{stellar}_\mathrm{ej,>5GK}$ ($N^\mathrm{stellar}_\mathrm{ej,>5GK}$) &  $M_\mathrm{>5GK}^\mathrm{inj}/M^\mathrm{inj}$\\
& ($10^{51}$\,erg) & ($M_\odot$) & ($10^{51}$\,erg) & ($10^3$\,km/s) &      & ($M_\odot$)      &  ($M_\odot$)      &  ($M_\odot$)  \\ 
\hline
AD009x0.5 &  0.59     &  0.56   &    0.26  &  6.67      &   38681 & 0.19 &  0.00 (     0) &  0.00 (     0)  &   0.39\\
AD015x0.5 &  2.51     &  1.49   &    0.93  &  7.79      &   4269 & 0.46 &  0.04 (   658) &  0.01 (   160)   &   0.44\\
AD017x0.5 &  2.81     &  1.52  &    0.91  &  7.61      &   43049 & 0.53 &  0.07 (  1105) &  0.01 (   111)   &   0.44\\
AD020x0.5 &  3.37     &  1.36   &    0.86  &  7.82      &   37600 & 0.51 &  0.12 (  2136) &  0.01 (   145)  &   0.46\\

\hline
AD009x0.6 &  0.93     &  0.78  &    0.35  &  6.72      &   52445 & 0.10 &  <0.01 (    10) &  0.00 (     1)  &   0.43\\
AD015x0.6 &  3.15     &  1.88   &    1.34  &  8.32      &   41193 & 0.64 &  0.06 (   787) &  0.02 (   187)  &   0.48\\
AD017x0.6 &  3.63     &  1.94   &    1.43  &  8.46      &   43309 & 0.65 &  0.12 (  1422) &  0.017 (   211)     &   0.48\\
AD020x0.6 &  4.67     &  1.77   &    1.35  &  8.61      &   39282 & 0.50 &  0.22 (  2799) &  0.01 (   165)  &   0.50\\
AD022x0.6 &  5.80     &  2.00   &    1.95  &  9.74      &   61595 & 0.75 &  0.34 (  4374) &  0.01 (   123)  &    0.52\\
AD025x0.6 &  6.22     &  1.85   &    1.60  &  9.17      &   43669 & 0.54 &  0.32 (  5047) &  0.02 (   249)  &   0.54\\

\hline
AD009x0.8 &  1.58     &  1.12   &    0.78  &  8.24      &   59195 & 0.20 &  <0.01 (    62) &  <0.01 (    12)    &   0.54\\
AD015x0.8 &  3.82     &  2.43   &    1.61  &  8.01      &   39308 & 0.78 &  0.09 (   799) &  0.02 (   208)  &   0.44\\
AD017x0.8 &  4.71     &  2.50   &    2.04  &  8.91      &   45816 & 0.83 &  0.19 (  1679) &  0.04 (   353)  &   0.52\\
AD020x0.8 &  6.45     &  2.28   &    1.98  &  9.20      &   42409 & 0.54 &  0.34 (  3419) &  0.03 (   277)  &   0.50\\
AD022x0.8 &  7.91     &  3.03   &    3.36  &  10.39     &   43355 & 1.20 &  0.58 (  4442) &  0.02 (   136)  &   0.55\\
AD025x0.8 &  9.77     &  2.82   &    3.13  &  10.63     &   89755 & 0.88 &  0.67 (  8515) &  0.02 (   138)  &   0.64\\
AD035x0.8 &  11.87    &  2.80   &    2.86  &  9.97      &   64595 & 1.11 &  0.80 (  7566) &  <0.01 (    24) &   0.55\\
\hline
AD009x1.0 & 2.03      &  1.39   &    1.11  &  8.82      &   45629 & 0.32 &  <0.01 (    84) &  <0.01 (     8)    &   0.64\\
AD015x1.0 & 4.21      &  2.37   &    1.37  &  7.50      &   41690 & 0.53 &  0.08 (   704) &  0.02 (   170)  &   0.45\\
AD017x1.0 & 5.21      &  3.07   &    2.21  &  8.36      &   40497 & 1.09 &  0.23 (  1634) &  0.05 (   344)  &   0.48\\
AD020x1.0 & 7.10      &  3.33   &    3.04  &  9.42      &   45856 & 1.23 &  0.46 (  2857) &  0.06 (   380)  &    0.52\\
AD022x1.0 & 9.05      &  3.61   &    3.97  &  10.28     &   49035 & 1.44 &  0.71 (  4340) &  0.04 (   278)  &   0.56\\
AD025x1.0 & 11.50     &  3.94   &    4.75  &  10.82     &   49748 & 1.52 &  0.95 (  5082) &  0.05 (   257)  &   0.59\\
AD030x1.0 & 13.46     &  4.40   &    5.16  &  10.68     &   55761 & 1.88 &  1.16 (  5597) &  0.02 (    57)  &   0.54\\
AD035x1.0 & 16.20     &  4.30  &    5.15  &  10.80     &   53789 & 1.70 &  1.24 (  6772) &  <0.01 (    28) &  0.56\\
AD040x1.0 & 17.55     &  3.73   &    3.38  &  9.37      &   38332 & 1.36 &  1.05 (  6878) &  0.10 (   663)  &   0.57\\
\hline
AD009x1.2 & 2.38      &  1.56   &    1.35  &  9.16      &   45537 & 0.39 &  0.01 (   162) &  <0.01 (    14)     &   0.65\\
AD015x1.2 & 4.19     &  2.98   &    1.74  &  7.52      &   62670 & 0.82 &  0.06 (   418) &  0.01 (    83)   &   0.45\\
AD017x1.2 & 5.55      &  3.28   &    2.25  &  8.17      &   39335 & 1.07 &  0.25 (  1536) &  0.04 (   294)  &   0.49\\
AD020x1.2 & 7.83      &  3.75   &    3.46  &  9.45      &   61895 & 1.24 &  0.48 (  2682) &  0.06 (   378)  &   0.53\\
AD022x1.2 & 9.77      &  4.07   &    4.16  &  9.96      &   72141 & 1.49 &  0.78 (  3882) &  0.08 (   381)  &   0.56\\
AD025x1.2 & 13.38     &  4.74   &    5.70  &  10.81     &   65685 & 1.72 &  1.02 (  4478) &  0.10 (   445)  &   0.58\\
AD030x1.2 & 15.00     &  5.27   &    6.19 &  10.84     &    &    &   &   &   \\
AD035x1.2 & 19.73     &  5.58   &    7.98  &  11.79     &   46960 & 2.21 &  1.73 (  5974) &  0.04 (   172)  &   0.55\\
AD040x1.2 & 22.86     &  5.64   &    8.15  &  11.82    &   58541 & 2.28 &  1.72 (  6033) &  0.017 (    34)  &   0.55\\
\hline
16TI      & 19.72     &  8.42   &    15.09  &  13.21   &  59430     & 1.14 & 0.008 (    25) &  0.0005 (     1)  & 0.67 \\
35OC     & 81.11     &  18.16  &     69.83  &  19.37   & 50626  &   3.031 &  0.3395 (   707) &  0.1812 (   383) & 0.75\\
\hline
\end{tabular}
\label{tab:models}
\end{table*}
